An Upper Bound of the Bias of Nadaraya-Watson Kernel Regression under Lipschitz Assumptions

The Nadaraya-Watson kernel estimator is among the most popular nonparameteric regression technique thanks to its simplicity. Its asymptotic bias has been studied by Rosenblatt in 1969 and has been reported in a number of related literature. However, Rosenblatt's analysis is only valid for infinitesimal bandwidth. In contrast, we propose in this paper an upper bound of the bias which holds for finite bandwidths. Moreover, contrarily to the classic analysis we allow for discontinuous first order derivative of the regression function, we extend our bounds for multidimensional domains and we include the knowledge of the bound of the regression function when it exists and if it is known, to obtain a tighter bound. We believe that this work has potential applications in those fields where some hard guarantees on the error are needed

==> BIOMETRIKA 2020 Arvix/sections/conclusion.tex <==
%\section{Conclusion}
%The Nadaraya--Watson kernel regression is one of the most well-known nonparametric estimator, used in a wide range of applications. His asymptotic bias and variance are well-known in the literature. However, to the best of our knowledge, the bias of such an estimator has never been bounded before.
%In this paper, we proposed a hard bound of the bias which requires mild assumptions. Our proposed bound is numerically tight and accurate for a large class of regression functions and random design. 
%We believe that providing hard, non-probabilistic, guarantees on the error of a regression algorithm is an important step for the adoption of data-driven algorithms in real world applications. Our future research will focus on extending the bias analysis to a wider class of kernel functions, and to allow for a finite samples analysis.

\section{Acknowledgment}
The research is financially supported by the Bosch-Forschungsstiftung program. 

%\section{Supplementary Material}
%Supplementary material available at \textsl{Biometrika} online includes the derivation of the theorems and the code used for the numerical simulation. 
%\blue{Let's do the conclusion together :).}

==> BIOMETRIKA 2020 Arvix/sections/preliminaries.tex <==

Consider the problem of estimating $\EV[Y | X= \xvec]$ where $X \sim f_X$ and $Y = m(X) + \epsilon$, with noise  $\epsilon$, i.e. $\EV[\epsilon] = 0$. The noise can depend on $\xvec$, but since our analysis is conducted point-wise for a given $\xvec$, $\epsilon_\xvec$ will be simply denoted by $\epsilon$. Let $m:\mathbb{R}^d\to \mathbb{R}$ be the \textsl{regression function} and $f_X$ a probability distribution on $X$ called \textsl{design}. In our analysis we consider $X \in \mathbb{R}^d$ and $Y \in \mathbb{R}$. 
The Nadaraya--Watson kernel estimate of $\EV[Y | X=\xvec]$ is 
\begin{align}
	\hat{m}(\xvec) = \frac{\sum_{i=1}^n K_{\hvec}(\xvec - \xvec_i) y_i}{\sum_{j=1}^n K_{\hvec}(\xvec - \xvec_j)},
\end{align} 
where $K_{\hvec}$ is a kernel function with bandwidth-vector $\hvec$, the $\xvec_i$ are drawn from the design $f_X$ and $y_i$ from $m(\xvec_i) + \epsilon$. Note that both the numerator and the denominator are proportional to Parzen-Rosenblatt density kernel estimates \citep{rosenblatt_remarks_1956,parzen_estimation_1962}.
We are interested in the point-wise bias of such estimate $\EV[\hat{m}(\xvec)]- m(\xvec)$. 
In the prior analysis of \cite{rosenblatt_conditional_1969}, knowledge of $m', m'', f_X, f_X'$ is required and $f, m'$ must be continuous in a neighborhood of $x$. In addition, and as discussed in the introduction, the analysis is limited to a one-dimensional design, and for an infinitesimal bandwidth. For clarity of exposition, we briefly present the classical bias analysis of \cite{rosenblatt_conditional_1969} before introducing our results. 
\begin{theorem}{\emph{Classic Bias Estimation \citep{rosenblatt_conditional_1969}.}}
	Let $m\!:\!\mathbb{R}\!\to\!\mathbb{R}$ be twice differentiable.
	Assume a set $\{x_i, y_i\}_{i=1}^n$ of i.i.d. samples from a distribution with non-zero differentiable density $f_X$. Assume $y_i = m(\svec_i) + \sigma(\epsilon_i)$, where $\epsilon_i$ are i.i.d. and zero-mean. The bias of the Nadaraya--Watson kernel in the limit of infinite samples and for $h \to 0$ and $nh_n \to \infty$ is 
	\begin{align}
	\EV \left[\lim_{n\to \infty}\approxx{m}_n(x) \right] - m(x)  & = h_n^2\left(\frac{1}{2}m''(x) + \frac{m'(x)f_X'(x)}{f_X(x)} \right)\int u^2 K(u)\de u + o_P\left(h_n^2\right) \nonumber \\
	& \approx h_n^2\left(\frac{1}{2}m''(x) + \frac{m'(x)f_X'(x)}{f_X(x)} \right)\int u^2 K(u)\de u . \nonumber
	\end{align}
\end{theorem}
The $o_P$ term denotes the asymptotic behavior w.r.t. the bandwidth. Therefore, for a larger value of the bandwidth, the bias estimation becomes worse, as is illustrated in Figure~\ref{figure:simulations}.

==> BIOMETRIKA 2020 Arvix/sections/simulation.tex <==
\begin{figure}[p]
	\includegraphics[width=\linewidth]{plots/figure_1.pdf}  
	\caption{\label{figure:simulations} 
		%In particular, we use $n=10^5$ samples to obtain $f_n$, and in order to obtain $\EV[f_n]$ we average on $100$ different estimates.
		\textsl{We propose some simulations of Nadaraya--Watson regression with different designs, regression functions and bandwidths.
			The regression function $m(x)$ is represented with a solid line, while the Nadaraya--Watson estimate $\hat{m}(x)$ is represented with a dash-dotted line in the top subplot of each experiment. 
			In the second subplots, it is possible to observe the true bias (solid line), as well as our upper bound (dashed line) and the Rosenblatt's estimate (dash-dotted line). 
			In the bottom subplots depict the design used.
			The bandwidth used for the estimation is denoted with $h$.
			It is possible to observe that the Rosenblatt's estimate  often under or over estimates the bias. In all the different test conditions, our method correctly upper bounds the bias.}
		%	In the first, second fourth and last plots, it is possible to observe that the bias is underestimated by the Rosenblatt's approach. In the first plot is also possible to observe that the Rosenblatt approach largely overestimate of the bias, as in $x=0$ the regression function has large second derivative.
		%	In the third plot, we used a small bandwidth, in order to highlight that is possible to obtain a tight bound and precise estimation of the bias with both the methods.
		%	The reader can observe that the proposed bound works for different choices of the design and regression functions.  
		%Our upper-bound is correct even close to the boundaries and for different design and regression functions, and has comparable magnitude of the Rosenblatt's.
	}
\end{figure}

In this section we provide a numerical analysis of our bounds on the bias.
We test our method on uni-dimensional input spaces for display purposes. We select a set of regression functions with different Lipschitz constants and different bounds,
\begin{itemize}
	\item $y = \sin(5x)$; $L_m = 5$ and $M=1$,
	\item $y = \log x$ which for $\mathcal{G} \equiv (-1, +\infty)$ has $L_m = 1$ and $M=+\infty$,
	\item $y = 60^{-1} \log\cosh 60 x $ which has $L_m=1$, is unbuounded, and has a particularly high second derivative in $x=0$, with $m''(0) = 60$,
	\item $y = \sqrt{x^2 + 1}$ which has $L_m = 1$ and is unbounded.  
\end{itemize}
In order to provide as many different scenarios as possible we also used the distributions from Table~\ref{table:distributions}, using therefore both infinite domain distributions, such as \textsl{Cauchy} and \textsl{Laplace}, and finite domain such as \textsl{Uniform}. 
In order to numerically estimate the bias, we approximate $E[\hat{m}_n(x)]$ with an ensemble of estimates $N^{-1}\sum_{j=1}^N\hat{m}_{n, j}(x)$ where each estimate $\hat{m}_{n,j}$ is built on a different dataset (drawn from the same distribution $f_X$). %\blue{what is jth dataset}. 
In order to ``simulate'' $n\to \infty$ we used $n=10^5$ samples. 

In this section we provide some simulations of our bound presented in Theorem~\ref{theo:bounded} and Theorem~\ref{theo:unbounded}, and for the Rosenblatt's case we use
\begin{equation}
	 \left| h_n^2\left(\frac{1}{2}m''(x) + \frac{m'(x)f_X'(x)}{f_X(x)} \right)\int u^2 K(u)\de u \right|\nonumber .
\end{equation}
Since the Rosenblatt's bias estimate is not an upper bound, it can happen that the true bias is higher (as well as lower) than this estimate, as it is possible to see in Figure~\ref{figure:simulations}. 
We presented different scenarios, both with bounded and unbounded functions, infinite and finite design domains, and with larger or smaller choice of bandwidths.
It is possible to observe that, thanks to the knowledge of $f, f', m', m''$ the Rosenblatt's estimation of the bias tends to be more accurate than our bound, however it can happen that it largely overestimate the bias, like in the case of $m(x) = 60^{-1}\log\cosh(60 x)$ in $x=0$ or to underestimate it, most often in boundary regions. 
In contrast, our bound always overestimate the true bias, and despite its lack of knowledge of $f, f', m', m''$, it is most often tight. Moreover, when the bandwidth is small, both our method and Rosenblatt's  deliver an accurate estimation of the bias.
In general, Rosenblatt tends to deliver a better estimate of the bias, but it does not behave as a bound, and in some situations it also can deliver larger mispredictions.
In detail, the plot (a) in Figure~\ref{figure:simulations} shows that, with a tight bandwidth both our method and Rosenblatt's method achieve good approximations of the bias, but only our method correctly upper bounds the bias.
When increasing the bandwidth, we obtain both a larger bias and subsequent larger estimates of the bias. Our method consistently upper bounds the bias, while in many cases Rosenblatt's method under estimates it, especially in proximity of boundaries (subplots b, d, e).
An interesting case can be observed in subplot (c), where we test the function $m(x) = 60^{-1}\log\cosh(60 x)$, which has high second order derivative in $x=0$: in this case, Rosenblatt's method largely overestimates the bias. 
%In detail, the plot (a) in Figure~\ref{figure:simulations}, shows that the Rosenblatt method both over- and lower-estimating the bias: the spike is given by a high second-order derivative of the regression function $m$ in $0$. Our proposed bound does not consider second derivatives and is still able to correctly bound the bias. In the subplots (b), (d) and (e) it is possible to see the Rosenblatt analysis underestimating the bias, particularly in proximity of the boundary. Plot (c) depicts a case where the bandwidth is small and both our method and Rosenblatt's achieve correct prediction of the bias.  
The figure shows that our bound is able to deal with different functions and random designs, being reasonably tight, if compared to the Rosenblatt's estimation which requires the knowledge of the regression function and the design, and respective derivatives.

==> BIOMETRIKA 2020 Arvix/sections/technical.tex <==
\begin{table}
	\begin{center}
		\begin{tabular}{||c c c c c||} 
			\hline
			Distribution & Density & $\Upsilon$ & $\mathcal{D}$ & $L_f$ \\ [0.5ex] 
			\hline\hline
			$\text{Laplace}(\mu, \lambda)$ & $\frac{1}{2\lambda}\exp{\left(-\frac{|x-\mu|}{\lambda}\right)}$& $(-\infty, +\infty)$ & $(-\infty, +\infty)$ & $\lambda^{-1}$  \\ 
			\hline
			$\text{Cauchy}(\mu; \gamma)$ & $\left(\pi\gamma + \pi\frac{(x-\mu)^2}{\gamma}\right)^{-1}$ & $(-\infty, +\infty)$ & $(-\infty, +\infty)$ & $\frac{2(z-\mu)}{\gamma^2+ (z-\mu)^2}$  \\
			\hline
			$\text{Uniform}(a, b)$ & $\begin{cases}
			\frac{1}{b-a} \quad \text{if} \quad a \leq x \leq b \\
			0 \quad \quad \text{otherwise}
			\end{cases}$ & $(a,b)$ & $(a,b)$ & 0 \\
			\hline
			$\text{Pareto}(\alpha)$ & $\begin{cases}
			\frac{\alpha}{x^{\alpha+1}} \quad \text{if}  x \geq 1 \\
			0 \quad \quad \text{otherwise}
			\end{cases}$ & $(1, +\infty)$ & $(1, +\infty)$ & $1+\alpha$ \\
			\hline
		    $\text{Normal}(\mu, \sigma)$ & $\frac{1}{\sqrt{2\pi\sigma^2}}\exp{-\frac{(x-\mu)^2}{2\sigma^2}}$ & $(-\infty, +\infty)$ & $(a, b)$ & $f_{\mu, \sigma}(a, b)$ \\
			\hline
		\end{tabular}
		
	\end{center}
	\caption{\label{table:distributions} \textsl{Examples of parameters to use for different univariate random design. Note that} $z = \frac{2\mu + \gamma^2 + \sqrt{4\mu + \gamma^4 + 2\mu\gamma^2 - 4(\gamma^2 + \mu + \gamma^2 \mu)}}{2}$ and in the case of the normal function one can find $f_{\mu, \sigma}(a,b) = \max_{y \in \{a, b\}} |\mathcal{N}(y | \mu, \sigma)|$.}
\end{table}
In this section we present two bounds on the bias of the Nadaraya--Watson estimator. The first one considers a bounded regression function $m$, and allows for local Lipschitz conditions on a subset of the design's support. The second bound instead does not require the regression function to be bounded but only the local Lipschitz continuity to hold on all of its support. The definition of ``local'' Lipschitz continuity will be given below. 

%\blue{do we need this? can't we just say here is a notation of an n-interval in Rd?}
In order to develop our bound on the bias for multidimensional inputs, it is important to define some subset of the $\mathbb{R}^d$ space. 
%More in detail we consider hyper-rectangles, called technically $d$-orthopodes. In our case, using such hyper-rectangle makes the computation of integrals easier. We define the $d$-orthopode as an open set, in order to allow the hyper-rectangle to be unbounded (for example a $2$-dimensional rectangle $(-\infty, +\infty)\times(-\infty, +\infty)$ is a valid orthopode).
More in detail we consider an open $n$-dimensional interval in $\mathbb{R}^d$ which is defined as $\Omega(\bm{\tau}^-, \bm{\tau}^+) \equiv (\tau_1^-, \tau_1^+) \times \dots  \times (\tau_d^-, \tau_d^+)$ where $\tau^-, \tau^+ \in \overline{\mathbb{R}}^d$.
%\begin{definition}{\emph{Open $d$-Orthopode.\\}}
%	Let a generic $d$-orthopode be a subset of $\mathbb{R}^d$ defined as an open interval $\Omega(\tau^-, \tau^+) \equiv (\tau_1, \tau_1^+) \times (\tau_2^-, \tau_2^+) \ \times \dots \times (\tau_d^-, \tau_d^+)$ where $\bm{\tau}^- = [\tau_1^-, \tau_2^-, \dots, \tau_d^-]^\intercal$, $\bm{\tau}^+ = [\tau_1^+, \tau_2^+, \dots, \tau_d^+]^\intercal$ with $\tau^-_i < \tau^+_i$.\blue{incomplete. are $\tau$ in R or extended R?}
%\end{definition}
We now formalize what is meant by weak (log-)Lipschitz continuity. This will prove useful as we need knowledge of the local-Lipschitz constants of $m$ and $\log f_X$ in our analysis. 
%http://imar.ro/journals/Mathematical_Reports/Pdfs/2007/3/miculescu.pdf
\begin{definition}{\emph{Weak Lipschitz continuity at $\xvec$ on the set $\mathcal{C}$ under the $L_1$-norm.\\}}
	Let $\mathcal{C} \subseteq \mathbb{R}^d$ and $f:\mathcal{C}\to \mathbb{R}$. We call $f$ weak Lipschitz continuous at $\xvec \in \mathcal{C}$ if and only if
	\begin{align}
		|f(\xvec) - f(\yvec)| \leq L|\xvec - \yvec|		\quad \forall \yvec \in \mathcal{C}, \nonumber 
	\end{align} 
	where $|\cdot|$ denotes the $L_1$-norm.
\end{definition}
\begin{definition}{\emph{Weak log-Lipschitz continuity at $\xvec$ on the set $\mathcal{C}$ under the $L_1$-norm.\\}}
	Let $\mathcal{C} \subseteq \mathbb{R}^d$. We call $f$ weak log-Lipschitz continuous at $\xvec$ on the set $\mathcal{C}$ if and only if
	\begin{align}
	|\log f(\xvec) - \log f(\yvec)| \leq L|\xvec - \yvec|		\quad \forall \yvec \in \mathcal{C} \nonumber .
	\end{align} 
	Note that the set $\mathcal{C}$ can be a subset of the function's domain.
\end{definition}
It is important to note that, in contrast to the global Lipschitz continuity, which requires 
$|f(\yvec) - f(\zvec)| \leq L |\yvec - \zvec|$ $\forall\yvec,\zvec \in \mathcal{C}$, the weak Lipschitz continuity is defined at a specific point $\xvec$ and therefore allows the function to be discontinuous elsewhere. 
In the following we list the set of assumptions that we use in our theorems.

% \blue{a5-a7... can we state these in the theorem instead?}
\begin{axioms}
	\item \label{ax:domain} $f_X$ and $m$ are defined on $\Upsilon \equiv \Omega(\xvec - \upsilon^-, \xvec + \upsilon^+)$ and  $\upsilon^-, \upsilon^+ \in \overline{\mathbb{R}}_+^d$%\blue{what is v?}
	\item \label{ax:log-lipschitz} $f_X$ is log weak Lipschitz with constant $L_f$ at $\xvec$ on the set $\mathcal{D} \equiv \Omega(\xvec -\deltab^-,\xvec + \deltab^- ) \subseteq \Upsilon$ and $f_X(\xvec) \geq f_X(\zvec)$ $\forall \zvec \in \Upsilon\backslash\mathcal{D}$ with positive defined $\deltab^-, \deltab^+ \in \overline{\mathbb{R}}_+^d$ (note that this implies $f_X(\yvec) > 0$ $\forall \yvec \in \mathcal{D}$), % \blue{where is the strict inq. coming from?}
	\item \label{ax:lipschitz} $m$ is weak Lipschitz with constant $L_m$ at $\xvec$ on a the set $\mathcal{G} \equiv \Omega(\xvec -\gammab^-, \xvec + \gammab^+) \subseteq \mathcal{D}$ with positive defined $\gammab^-, \gammab^+ \in \overline{\mathbb{R}}_+^d$,
	%\item \label{ax:x} $\xvec \in \mathcal{G}$, \blue{can we avoid this from A3?}
%	\item \label{ax:bandwidth} 	$\hvec \in \mathbb{R}^{d}$ is a positive defined vector of bandwidths $\hvec = [h_1, h_2, \dots, h_n]^\intercal$, and $K_h$ be the multivariate Gaussian kernel defined on $\hvec$,
%	\item \label{ax:noise}  $\hat{f}_n(\xvec)$ is the Nadaraya-Watson kernel estimate using $n$ observations $\{\xvec_i, y_i\}_{i=1}^n$  with $x_i \sim f_X$, $y_i = m(\xvec_i) + \epsilon_i$ with $\epsilon_i \sim \varepsilon(\xvec_i)$ and $\EV[\varepsilon(\xvec_i)] = 0$,
%	\item \label{ax:infinitesamples} the number of samples considered tends to infinite, $n\to \infty$,
%	\item \label{ax:maximum} There is a constant $0\leq M < +\infty$  such that $|m(\yvec) - x(\zvec)| \leq M$ $\forall \yvec, \zvec \in \Upsilon$.
\end{axioms}

In the following, we propose two different bounds of the bias. The first version considers a bounded regression function ($M < +\infty$), this allows both the regression function and the design to be weak Lipschitz on a subset of their domain. 
In the second version instead, we consider the case of unbounded regression function ($M = +\infty$) or when the bound $M$ is not known. In this case both the regression function and the design must be weak Lipschitz on the entire domain $\Upsilon$. 
\begin{theorem}{\emph{Bound on the Bias with Bounded Regression Function.}\\}
	\label{theo:bounded}
	Assuming \ref{ax:domain}--\ref{ax:lipschitz}, $\hvec \in \mathbb{R}^{d}_+$ a positive defined vector of bandwidths $\hvec = [h_1, h_2, \dots, h_n]^\intercal$, $K_h$ a multivariate Gaussian kernel defined on $\hvec$, $\hat{f}_n(\xvec)$ the Nadaraya--Watson kernel estimate using $n$ observations $\{\xvec_i, y_i\}_{i=1}^n$  with $x_i \sim f_X$, $y_i = m(\xvec_i) + \epsilon_i$ and with noise $\epsilon_i \sim \varepsilon(\xvec_i)$ centered in zero ($\EV[\varepsilon(\xvec_i)] = 0$), $n\to \infty$, and furthermore assuming there is a constant $0\leq M < +\infty$  such that $|m(\yvec) - x(\zvec)| \leq M$ $\forall \yvec, \zvec \in \Upsilon$, the considered Nadaraya--Watson kernel regression bias results to be bounded by 
	\begin{align}
	& \bigg|\EV\Big[\lim_{n\to \infty}\approxx{f}_n(\xvec) \Big] - m(\xvec)\bigg|\nonumber \\
	& \leq \frac{\sum\limits_{k=1}^d {\xi_A}_k \prod\limits_{i\neq k}^d  \zeta(h_i, -\phi_i^-, \phi_i^+)+ M\left(\prod\limits_{i=1}^d\zeta(-\gamma_i^-, \gamma_i^+)  -  \prod\limits_{i=1}^d\zeta(-\phi_i^-, \phi_i^+)+ \prod\limits_{i=1}^d2{\xi_C}_i \right)}{\prod_{i=1}^d \Psi(L_f, h_i, -\delta_i^-, \delta_i^+)} \nonumber
	\end{align}
	where \begin{align}
	& {\xi_A}_k  = \frac{\sqrt{2}L_m h_k}{\sqrt{\pi}} \left(2 - \phi(\phi_k^+, -L_f, h_k)- \phi(-\phi_k^-, L_f, h_k)\right) - L_mL_fh_k^2\zeta(h_k, -\phi_k^-, \phi_k^+) \nonumber, \\
	& \zeta(h, \tau^-, \tau^+) = \e{\frac{L_f^2 h^2}{2}}\left( 2 \varphi(0, L_f, h) - \varphi(-\tau^+, L_f, h) - \varphi(\tau^-, L_f, h)\right) \nonumber,\\
	& \Psi(L, h, \tau^-, \tau^+) = e^{\frac{L^2h^2}{2}}\left(\varphi(\tau^+, L, h) - \varphi(\tau^-, L, h)\right) \nonumber, \\
	& \varphi(l, L, h) = \lim_{g\to l}\erf\left(\frac{g + h^2L}{h\sqrt{2}} \right),  
	\phi(l, L, h) = \lim_{g\to l} e^{-\frac{g^2}{2h^2} - g L} \nonumber
	\end{align}
	$ \phi_i^-=-M/L_m, \phi_i^+=M/L_m$ and $\erf$ is the error function.
\end{theorem}
In the case where $M$ is unknown or infinite, we propose the following bound.
\begin{theorem}{\emph{Bound on the Bias with Unbounded Regression Function.}\\}
	\label{theo:unbounded}
	Assuming \ref{ax:domain}--\ref{ax:lipschitz}, $\hvec \in \overline{\mathbb{R}}_+^{d}$ a positive defined vector of bandwidths $\hvec = [h_1, h_2, \dots, h_n]^\intercal$, $K_h$ a multivariate Gaussian kernel defined on $\hvec$, $\hat{f}_n(\xvec)$ the Nadaraya--Watson kernel estimate using $n$ observations $\{\xvec_i, y_i\}_{i=1}^n$  with $x_i \sim f_X$, $y_i = m(\xvec_i) + \epsilon_i$ and with noise $\epsilon_i \sim \varepsilon(\xvec_i)$ centered in zero ($\EV[\varepsilon(\xvec_i)] = 0$), $n\to \infty$, and furthermore assuming that $\Upsilon \equiv \mathcal{D} \equiv \mathcal{G}$, the considered Nadaraya--Watson kernel regression bias results to be bounded by
	\begin{align}
	   & \bigg|\EV\Big[\lim_{n\to \infty}\approxx{f}_n(\xvec) \Big] - m(\xvec)\bigg|  \leq \frac{\sum\limits_{k=1}^d {\xi_A}_k\prod\limits_{i\neq k}^d  \zeta(h_i, -\upsilon_i^-, \upsilon_i^+)}{\prod_{i=1}^d \Psi(L_f, h_i, -\upsilon_i^-, \upsilon_i^+)} \nonumber
	   \end{align}
	   where $\xi_{A_k}, \zeta, \Psi, \varphi$ are defined as in Theorem~\ref{theo:bounded} and $\phi_i^-=\upsilon_i^-, \phi_i^+=\upsilon_i^+$.
\end{theorem}

	
The proof of both theorems is detailed in the Supplementary Material.
Note that the conditions required by our theorems are mild and they allow a wide range of random designs, including and not limited to Gaussian, Cauchy, Pareto, Uniform and Laplace distributions. In general every continuously differentiable density distribution is also weak log-Lipschitz in some closed subset of its domain. For example, the Gaussian distribution does not have a finite Lipschitz constant on its entire domain, but on any closed interval, there is a finite weak Lipschitz constant. Examples of densities that are weak log-Lipschitz are presented in Table~\ref{table:distributions}.




